Continious-time Importance Sampling: Monte Carlo Methods which Avoid Time-discretisation Error

In this paper we develop a continuous-time sequential importance sampling (CIS) algorithm which eliminates time-discretisation errors and provides online unbiased estimation for continuous time Markov processes, in particular for diffusions. Our work removes the strong conditions imposed by the EA and thus extends significantly the class of discretisation error-free MC methods for diffusions. The reason that CIS can be applied more generally than EA is that it no longer works on the path space of the SDE. Instead it uses proposal distributions for the transition density of the diffusion, and proposal distributions that are absolutely continuous with respect to the true transition density exist for general SDEs.

==> deriv.tex <==
\section{Intuitive derivation: CIS as a limiting algorithm}
\label{S:deriv}

In this section we illustrate an intuitive derivation of the CIS
algorithm as the limiting algorithm of a standard discrete-time
sequential importance sampler.

\subsection*{Standard Sequential Importance Sampling}

We will now describe a standard discrete-time sequential importance
sampler \citep{kong:liu:1994}. Firstly discretise the time interval
$[0,\th]$ into intervals of length $h$. The sequential importance
sampler will simulate values of the process and importance weights at
times $h,2h,\ldots$. If at time $\ci$ we have a value and weight,
$\xx{\ci},\ww{\ci}$, then we first generate $\xx{\ni}$ from
$\prd{\xx{\ci}}{\cdot}{h}{\theta_{k-1}}$ and set
$$w_{\ni}=w_{\ci}\trd{\xx{\ci}}{\xx{\ni}}{h}/\prd{\xx{\ci}}{\xx{\ni}}{h}{\theta_{k-1}}.$$ 
Full details are given in Algorithm \algsis.

\begin{description}

\item[{\bf Algorithm \algsis}:] {\it Discrete-time Sequential Importance Sampler} (SIS).

\item[{\it Input}:] $\th$ a time to stop, $M$ a discretisation level and
  $\xx{0}$ the initial value.

\item[{\it Initialise}:] Set $w_0=1$ and $h=\th/M$.
  
\item[{\it Iterate}:] For $1\leq \myi\leq M$
    \begin{enumerate}
    \item choose $\theta_{k-1}$ and draw $\xx{\ni}\sim \prd{\xx{\ci}}{\cdot}{h}{\theta_{\myi-1}}$,
    \item update the weight
      \[
      w_{\ni}=w_{\ci}\frac{\trd{\xx{\ci}}{\xx{\ni}}{h}}{\prd{\xx{\ci}}{\xx{\ni}}{h}{\theta_{\myi-1}}}.
      \]
    \end{enumerate}
  
\end{description}

Let $X_{\myi h},W_{\myi h}$ denote the random variables of the value and
weight at time $\myi h$, respectively. Standard importance sampling
arguments show that whenever the left-hand side is defined, then
% 
\begin{equation} \label{eq:2}
\mbox{E}_p[f(X_{\myi h})]=\mbox{E}_q[W_{\myi h}f(X_{\myi h})],
\end{equation}
% 
where $\mbox{E}_q$ denotes expectation of $X_{\myi h},W_{\myi h}$ with
respect to the sequential importance sampling process.

Unfortunately Algorithm {\algsis} cannot be implemented
since $\trd{x}{\y}{h}$ is unknown, hence the weights cannot be
updated at each iteration. To overcome this, the aim is to consider
the limit as $h\rightarrow 0$, which however cannot be considered at
this point as such a limit would not make sense. So first we adapt
Algorithm {\algsis} using in turn ideas of random weight sequential importance
sampling \citep{fear:papa:robe:2008},
retrospective sampling \citep{papa:robe:2008} and
Rao-Blackwellisation \cite[]{liu:chen:1998}.

\subsection*{Random Weight sequential Importance Sampling}

Our first idea is to change how the weights are updated, and to make
this update random. This will still produce a valid importance
sampler, for which (\ref{eq:2}) is satisfied, provided that the mean
of the random weight update is equal to the true incremental weight.

We will implement our random weight update by introducing a series of
Bernoulli random variables, $U_{\myi h}$, for $\myi =1,2,\ldots$.  We call
successes of the Bernoulli random variables, events. We will allow the
distribution of $U_{\myi h}$ to depend on the time $\myi h$ and also the
history of the Bernoulli process, but for concreteness and notational
simplicity we will consider only the case where it depends on the time
since the most recent event has occurred. That is, if the most recent
event has happened at time $jh$, then we assume there exists a
function $\lambda(\cdot)>0$ such that with probability
$h\lambda(\ni-jh)$, $U_{\ni}=1$, otherwise $U_{\ni}=0$. It is trivial to
see that if
\begin{align*}
\rw{x}{\y}{h}{u}{\theta}:=1+\frac{1}{h\lambda(u)}\left\{\frac{\trd{x}{y}{h}}{\prd{x}{\y}{h}{\theta}}-1\right\},
% r(x_{(i-1)h},x_{ih},h,\theta_i,ih-jh)=1+\frac{1}{h\lambda(ih-jh)}\left\{\frac{\trd{x_{(i-1)h}}{x_{ih}}{h}}{\prd{x_{(i-1)h}}{x_{ih}}{h}{\theta_i}}-1\right\},
\end{align*}
%
then
% 
\begin{align*}
  \frac{\trd{\xx{\ci}}{\xx{\ni}}{h}}{\prd{\xx{\ci}}{\xx{\ni}}{h}{\theta_{\myi-1}}}=\mbox{E}\lsb
    (1-U_{\ni})+U_{\ni}\rw{\xx{\ci}}{\xx{\ni}}{h}{(\myi-j)h}{\theta_{\myi-1}}\rsb.
\end{align*}
% 
Thus, we can define an appropriate random incremental weight that
takes the value $1$ if $U_{\myi h}=0$ and
$\rw{x_{\ci}}{x_{\ni}}{h}{(\myi-j)h}{\theta_{\myi-1}}$ if $U_{\ni}=1$. The
resulting algorithm is shown in Algorithm {\algrwsis}.

\begin{description}

\item[{\bf Algorithm \algrwsis}:] {\it Random weight SIS}.

\item[{\it Input}:] $\th$ a time to stop, $M$ a discretisation level and $\xx{0}$ the initial value.

\item[{\it Initialise}:] Set $\ww{0}=1,\, h=\th/M$ and $j=0$.
  
\item[{\it Iterate}:] For $1\leq \myi\leq M$
  \begin{enumerate}
  \item choose $\theta_{\myi-1}$ and draw $\xx{\ni}\sim
    \prd{\xx{\ci}}{\cdot}{h}{\theta_{\myi-1}}$,
    
  \item draw $U_{\ni}$, a Bernoulli random variable with success
    probability $ h\lambda(\myi h-jh)$,
    
  \item if $U_{\ni}=1$, set
      \[
      \ww{\ni}=\ww{\ci}\rw{\xx{\ci}}{\xx{\ni}}{h}{(\myi-j)h}{\theta_{\myi-1}},
      \]
      and $j=\myi$; else set $w_{\ni}=w_{\ci}$.
  \end{enumerate}
  
\end{description}


\subsection*{Retrospective Sampling and Rao-Blackwellisation}

Algorithm {\algrwsis} cannot be implemented in practice, as the random
incremental weights still depend on the unknown transition density of
the proposal process. Furthermore, even if it could be implemented, it
would be less efficient than Algorithm {\algsis} because of the extra
randomness introduced by the random variables
$U_{\myi h},\,\myi=1,2,\ldots$. However its use is that it now enables us to
use the ideas of Retrospective Sampling and then Rao-Blackwellisation.

The idea behind Retrospective Sampling is to interchange the order of
simulating $\xx{\myi h}$ and $U_{\myi h}$, and to note that if
$U_{\myi h}=0$ then we do not need to simulate $\xx{\myi h}$ at all. So we
will only simulate $\xx{\myi h}$ at time points when there is an event. If
$jh$ is the time of the most recent event prior to $\myi h$, then
$\xx{\myi h}$ is simulated from the proposal transition density
$\prd{x_{jh}}{\cdot}{(\myi-j)h}{\theta_j}$. To update the weight at time
$\ni$ we also need to know the value of $\xx{\ci}$ and so this has
to be simulated, conditionally on $\xx{jh}$ and $\xx{\ni}$, from the
density
% 
\begin{equation} \label{eq:xi-1}
q(\xx{\ci}\mid x_{jh},x_{\ni}):=\frac{\prd{\xx{jh}}{\xx{\ci}}{(\myi-j-1)h}{\theta_j}\prd{\xx{\ci}}{\xx{\ni}}{h}{\theta_j}}{\prd{\xx{jh}}{\xx{\ni}}{(\myi-j)h}{\theta_j}}.
\end{equation}
% 
This can be viewed as introducing a random incremental weight. The
weight depends on the value of $\xx{\ci}$ that is simulated. The
idea behind Rao-Blackwellisation is that a more efficient algorithm
can be produced by replacing this random incremental weight by a
deterministic one that is equal to the mean of the random incremental
weight. We denote this mean by
% 
\begin{align*} 
  \mrwh{\xx{jh}}{\xx{\ni}}{h}{(\myi-j)h}{\theta_j}=\int
  \rw{\y}{\xx{\ni}}{h}{(\myi-j)h}{\theta_j}q(\xx{\ci}\mid \xx{jh},\xx{\ni})
  \d\y.
\end{align*}
% 
The resulting algorithm is given in detail in Algorithm
\algrbsis. Note if we stop the algorithm at a time point at which
there is no event, then the weight at that time is equal to the value
of the weight at the last event time, and the value of the process can
be simulated from the appropriate transition density of the proposal
process given the time and value at the last event time.

\begin{description}

\item[{\bf Algorithm \algrbsis}:] {\it SIS with Retrospective Sampling and Rao-Blackwellisation}.

\item[{\it Input}:] $\th$ a time to stop, $M$ a discretisation level and $\xx{0}$ the initial value.

\item[{\it Initialise}:] Set $w_0=1,\, h=\th/M,\,j=0$ and choose $\theta_j$.
  
\item[{\it Iterate}:] For $1\leq \myi\leq M$
  \begin{enumerate}
    
  \item draw $U_{\ni}$, a Bernoulli random variable with success
    probability $ h\lambda(\ni-jh)$,

  \item if $U_{\ni}=1$, then
    \begin{enumerate}
    \item draw $\xx{\ni}\sim
    \prd{\xx{jh}}{\cdot}{h}{\theta_j}$,
  \item update the weight
    \begin{align*}
      w_{\ni}=w_{\ci}\,\mrwh{\xx{jh}}{\xx{\ni}}{h}{(\myi-j)h}{\theta_j},
    \end{align*}
  \item set $j=\myi$ and choose $\theta_j$.
    \end{enumerate}
  \end{enumerate}
  
\end{description}


\subsection*{CIS as a limiting algorithm}

Whilst Algorithm {\algrbsis} cannot be implemented, we can now take
the limit as $h\rightarrow0$. In doing this the Bernoulli random
variables will converge to a renewal process with rate of an event at
a time $\tau$ since the last event being $\lambda(\tau)$. We will thus
obtain a limiting algorithm where events are simulated from a Poisson
process, the value of the process at these events are drawn from the
proposal transition density, and the weights are updated based on the
simulated value. The key thing is that in this limit the incremental
weight is tractable. If we fix $s=jh$ and $t=kh$ and let $h\rightarrow
0$, then
% 
\begin{align*}
  &\lim_{h\rightarrow 0}
  \mrwh{\xx{s}}{\xx{t}}{h}{t-s}{\theta_s}=\\
% 
&= 1 + \frac{1}{\lambda(t-s)} \lim_{h\rightarrow 0} \int
\frac{1}{h}\left\{\frac{\prd{x_{s}}{\y}{t-s-h}{\theta_s}[\trd{\y}{x_{t}}{h}-\prd{\y}{x_{t}}{h}{\theta_s}]}{\prd{x_{s}}{x_{t}}{t-s}{\theta_s}}\right\}\mbox{d}\y.
\end{align*}
% 
However by integrating (\ref{eq:PDE}) over a time interval of length
$h$, with an initial distribution for the process being $
\prd{x_{s}}{\y}{t-s-h}{\theta_s}$ we get:
% 
\begin{align*} \int
  \prd{x_{s}}{\y}{t-s-h}{\theta_s}\trd{\y}{x_{t}}{h}\mbox{d}\y &=
  \prd{x_{s}}{x_t}{t-s-h}{\theta_s} \\
  &+ h \tro\prd{x_{s}}{x_t}{t-s-h}{\theta_s}+o(h),
\end{align*}
% 
and similarly for the term which involves
$\prd{\y}{x_t}{h}{\theta_s}$. Thus
% 
\begin{align*} 
  \lim_{h\rightarrow 0} \mrwh{\xx{s}}{\xx{t}}{h}{t-s}{\theta_s}
  = 1+\frac{\lsb\tro-\prot{\theta_s} \rsb
    \prd{x_{s}}{\y}{t-s}{\theta_s}|_{\y=x_t}}{\lambda(t-s)\prd{x_{s}}{x_{t}}{t-s}{\theta_s}}.
\end{align*}
% 
which is exactly the incremental weight \eqref{eq:iweight} used in the CIS algorithm.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> derivation.tex <==
\section{Intuitive derivation: CIS as a limiting algorithm}

In this section we illustrate an intuitive derivation of the CIS
algorithm as the limiting algorithm of a standard discrete-time
sequential importance sampler.

\subsection*{Standard Sequential Importance Sampling}

We will now describe a standard discrete-time sequential importance
sampler \citep{kong:liu:1994}. Firstly discretise the time interval
$[0,\th]$ into intervals of length $h$. The sequential importance
sampler will simulate values of the process and importance weights at
times $h,2h,\ldots$. If at time $(i-1)h$ we have a value and weight,
$x_{(i-1)h},w_{(i-1)h}$, then we first generate $x_{ih}$ from
$\prd{x_{(i-1)h}}{\cdot}{h}{\theta_{i-1}}$ and set
$$w_{ih}=w_{(i-1)h}\trd{x_{(i-1)h}}{x_{ih}}{h}/\prd{x_{(i-1)h}}{x_{ih}}{h}{\theta_{i-1}}.$$ 
We refer to the term
$\trd{x_{(i-1)h}}{x_{ih}}{h}/\prd{x_{(i-1)h}}{x_{ih}}{h}{\theta_{i-1}}$
as the {\em incremental weight}. Full details are given in Algorithm
\algsis.

\begin{description}

\item[{\bf Algorithm \algsis}:] {\it Discrete-time Sequential Importance Sampler} (SIS).

\item[{\it Input}:] $T$ a time to stop, $M$ a discretisation level and
  $x_0$ the initial value.

\item[{\it Initialise}:] Set $w_0=1$ and $h=T/M$.
  
\item[{\it Iterate}:] For $1\leq i\leq M$
    \begin{enumerate}
    \item choose $\theta_{i-1}$ and draw $x_{ih}\sim \prd{x_{(i-1)h}}{\cdot}{h}{\theta_{i-1}}$,
    \item update the weight
      \[
      w_{ih}=w_{(i-1)h}\frac{\trd{x_{(i-1)h}}{x_{ih}}{h}}{\prd{x_{(i-1)h}}{x_{ih}}{h}{\theta_{i-1}}}.
      \]
    \end{enumerate}
  
\end{description}

% \begin{algorithm}[ht]
%   \begin{footnotesize}
%     \rule{\textwidth}{1mm}
%     \underline{Discrete-time SIS}

%     \begin{tabular}[h]{ll}
%       {\bf Initialise:} & Set $X_0=x_0$, and $w_0=1$.
%       \\
%       \\ 
%     \end{tabular}

%     {\bf Iterate:} For $i=1,2,\ldots$
%     \begin{enumerate}
%     \item Choose an appropriate $\theta_i$ value.
%     \item Simulate $X_{ih}=x_{ih}$, drawn from $q(x_{(i-1)h},x_{ih},h;\theta_i)$.
%     \item Update the weight:
%       \[
%       w_{ih}=w_{(i-1)h}\frac{p(x_{(i-1)h},x_{ih},h)}{q(x_{(i-1)h},x_{ih},h;\theta_i)}.
%       \]
%     \end{enumerate}
%     \rule{\textwidth}{1mm}
%     \caption{\footnotesize Discrete-time Sequential Importance Sampler (SIS). \label{Alg:1}}
%   \end{footnotesize}
% \end{algorithm}

Let $X_{ih},W_{ih}$ denote the random variables of the value and
weight at time $ih$, respectively. Standard importance sampling
arguments show that whenever the left-hand side is defined, then
% 
\begin{equation} \label{eq:2}
\mbox{E}_p[f(X_{ih})]=\mbox{E}_q[W_{ih}f(X_{ih})],
\end{equation}
% 
where $\mbox{E}_p$ denotes expectation of $X_{ih}$ with respect to the
target process, and $\mbox{E}_q$ expectation of $X_{ih},W_{ih}$ with
respect to the sequential importance sampling process.

Unfortunately Algorithm {\algsis} cannot be implemented
since $\trd{x}{\y}{h}$ is unknown, hence the weights cannot be
updated at each iteration. To overcome this, our aim is to consider
the limit as $h\rightarrow 0$, which however cannot be considered at
this point as such a limit would not make sense. So first we adapt
Algorithm {\algsis} using in turn ideas of random weight sequential importance
sampling \citep{fear:papa:robe:2008},
retrospective sampling \citep{papa:robe:2008} and
Rao-Blackwellisation \cite[]{liu:chen:1998}.

\subsection*{Random Weight sequential Importance Sampling}

Our first idea is to change how the weights are updated, and to make
this update random. This will still produce a valid importance
sampler, for which (\ref{eq:2}) is satisfied, provided that the mean
of the random weight update is equal to the true incremental weight.

We will implement our random weight update by introducing a series of
Bernoulli random variables, $U_{ih}$, for $i=1,2,\ldots$.  We call
successes of the Bernoulli random variables, events. We will allow the
distribution of $U_{ih}$ to depend on the time $ih$ and also the
history of the Bernoulli process, but for concreteness and notational
simplicity we will consider only the case where it depends on the time
since the most recent event has occurred. That is, if the most recent
event has happened at time $jh$, then we assume there exists a
function $\lambda(\cdot)>0$ such that with probability
$h\lambda(ih-jh)$, $U_{ih}=1$, otherwise $U_{ih}=0$. It is trivial to
see that if
\begin{align*}
\rw{x}{\y}{h}{u}{\theta}:=1+\frac{1}{h\lambda(u)}\left\{\frac{\trd{x}{y}{h}}{\prd{x}{\y}{h}{\theta}}-1\right\},
% r(x_{(i-1)h},x_{ih},h,\theta_i,ih-jh)=1+\frac{1}{h\lambda(ih-jh)}\left\{\frac{\trd{x_{(i-1)h}}{x_{ih}}{h}}{\prd{x_{(i-1)h}}{x_{ih}}{h}{\theta_i}}-1\right\},
\end{align*}
%
then
% 
\begin{align*}
  \frac{\trd{x_{(i-1)h}}{x_{ih}}{h}}{\prd{x_{(i-1)h}}{x_{ih}}{h}{\theta_{i-1}}}=\mbox{E}\lsb
    (1-U_{ih})+U_{ih}\rw{x_{(i-1)h}}{x_{ih}}{h}{(i-j)h}{\theta_{i-1}}\rsb.
\end{align*}
% 
Thus, we can define an appropriate random incremental weight that
takes the value $1$ if $U_{ih}=0$ and
$\rw{x_{(i-1)h}}{x_{ih}}{h}{(i-j)h}{\theta_{i-1}}$ if $U_{ih}=1$. The
resulting algorithm is shown in Algorithm {\algrwsis}.

\begin{description}

\item[{\bf Algorithm \algrwsis}:] {\it Random weight SIS}.

\item[{\it Input}:] $T$ a time to stop, $M$ a discretisation level and $x_0$ the initial value.

\item[{\it Initialise}:] Set $w_0=1,\, h=T/M$ and $j=0$.
  
\item[{\it Iterate}:] For $1\leq i\leq M$
  \begin{enumerate}
  \item choose $\theta_{i-1}$ and draw $x_{ih}\sim
    \prd{x_{(i-1)h}}{\cdot}{h}{\theta_{i-1}}$,
    
  \item draw $U_{ih}$, a Bernoulli random variable with success
    probability $ h\lambda(ih-jh)$,
    
  \item if $U_{ih}=1$, set
      \[
      w_{ih}=w_{(i-1)h}\rw{x_{(i-1)h}}{x_{ih}}{h}{(i-j)h}{\theta_{i-1}},
      \]
      and $j=i$; else set $w_{ih}=w_{(i-1)h}$.
  \end{enumerate}
  
\end{description}

% \begin{algorithm}[ht]
%   \begin{footnotesize}
%     \rule{\textwidth}{1mm}
%     \underline{Random weight SIS}

%     \begin{tabular}[h]{ll}
%       {\bf Initialise:} & Set $X_0=x_0$, $w_0=1$ and $j=1$.
%       \\
%       \\ 
%     \end{tabular}

%     {\bf Iterate:} For $i=1,2,\ldots$
%     \begin{enumerate}
%     \item Choose an appropriate $\theta_i$.
%     \item Simulate $X_{ih}=x_{ih}$, drawn from $q(x_{(i-1)h},x_{ih},h;\theta_i)$.
%     \item Simulate a realisation of $U_{ih}$, a Bernoulli random variable with success probability $
%       h\lambda(ih-jh)$.
%     \item If $U_{ih}=1$, set
%       \[
%       w_{ih}=w_{(i-1)h}r(x_{(i-1)h},x_{ih},h,\theta,ih-jh),
%       \]
%       and $j=i$; otherwise set $w_{ih}=w_{(i-1)h}$.
%     \end{enumerate}
%     \rule{\textwidth}{1mm}
%     \caption{\footnotesize Random weight SIS. \label{Alg:2}}
%   \end{footnotesize}
% \end{algorithm}


\subsection*{Retrospective Sampling and Rao-Blackwellisation}

Algorithm {\algrwsis} cannot be implemented in practice, as the random
incremental weights still depend on the unknown transition density of
the proposal process. Furthermore, even if it could be implemented, it
would be less efficient than Algorithm {\algsis} because of the extra
randomness introduced by the random variables
$U_{ih},\,i=1,2,\ldots$. However its use is that it now enables us to
use the ideas of Retrospective Sampling and then Rao-Blackwellisation.

The idea of Retrospective Sampling is to interchange the order of
simulating $x_{ih}$ and $U_{ih}$, and to note that if $U_{ih}=0$ then
we do not need to simulate $x_{ih}$ at all. So we will only simulate
$x_{ih}$ at time points when there is an event. If $jh$ is the time
of the most recent event prior to $ih$, then $X_{ih}$ is simulated
from the proposal transition density
$\prd{x_{jh}}{\cdot}{(i-j)h}{\theta_j}$. To update the weight at time
$ih$ we also need to know the value of $X_{(i-1)h}$ and so this has to
be simulated, conditionally on $x_{jh}$ and $x_{ih}$, from the
density
% 
\begin{equation} \label{eq:xi-1}
q(x_{(i-1)j}\mid x_{jh},x_{ih}):=\frac{\prd{x_{jh}}{x_{(i-1)h}}{(i-j-1)h}{\theta_j}\prd{x_{(i-1)h}}{x_{ih}}{h}{\theta_j}}{\prd{x_{jh}}{x_{ih}}{(i-j)h}{\theta_j}}.
\end{equation}
% 
This can be viewed as introducing a random incremental weight. The
weight depends on the value of $x_{(i-1)h}$ that is simulated. The
idea behind Rao-Blackwellisation is that a more efficient algorithm
can be produced by replacing this random incremental weight by a
deterministic one that is equal to the mean of the random incremental
weight. We denote this mean by
% 
\begin{align*} 
  \mrwh{x_{jh}}{x_{ih}}{h}{(i-j)h}{\theta_j}=\int
  % \rw{\y}{x_{ih}}{h}{(i-j)h}{\theta_j}\frac{\prd{x_{jh}}{\y}{(i-j-1)h}{\theta_j}\prd{\y}{x_{ih}}{h}{\theta_j}}{\prd{x_{jh}}{x_{ih}}{(i-j)h}{\theta_j}}
  \rw{\y}{x_{ih}}{h}{(i-j)h}{\theta_j}q(x_{(i-1)j}\mid x_{jh},x_{ih})
  \d\y.
\end{align*}
% 
The resulting algorithm is given in detail in Algorithm
\algrbsis. Note if we stop the algorithm at a time point at which
there is no event, then the weight at that time is equal to the value
of the weight at the last event time, and the value of the process can
be simulated from the appropriate transition density of the proposal
process given the time and value at the last event time.

\begin{description}

\item[{\bf Algorithm \algrbsis}:] {\it SIS with Retrospective Sampling and Rao-Blackwellisation}.

\item[{\it Input}:] $T$ a time to stop, $M$ a discretisation level and $x_0$ the initial value.

\item[{\it Initialise}:] Set $w_0=1,\, h=T/M,\,j=0$ and choose $\theta_j$.
  
\item[{\it Iterate}:] For $1\leq i\leq M$
  \begin{enumerate}
    
  \item draw $U_{ih}$, a Bernoulli random variable with success
    probability $ h\lambda(ih-jh)$,

  \item if $U_{ih}=1$, then
    \begin{enumerate}
    \item draw $x_{ih}\sim
    \prd{x_{jh}}{\cdot}{h}{\theta_j}$,
  \item update the weight
    \begin{align*}
      w_{ih}=w_{(i-1)h}\,\mrwh{x_{jh}}{x_{ih}}{h}{(i-j)h}{\theta_j},
    \end{align*}
  \item set $j=i$ and choose $\theta_j$.
    \end{enumerate}
  \end{enumerate}
  
\end{description}

% \begin{algorithm}[ht]
%   \begin{footnotesize}
%     \rule{\textwidth}{1mm}
%     \underline{SIS with Retrospective Sampling and Rao-Blackwellisation.}

%     \begin{tabular}[h]{ll}
%       {\bf Initialise:} & Set $X_0=x_0$, $w_0=1$ and $j=1$; and choose $\theta_0$.
%       \\
%       \\ 
%     \end{tabular}

%     {\bf Iterate:} For $i=1,2,\ldots$
%     \begin{enumerate}
%     \item Simulate a realisation of $U_{ih}$, a Bernoulli random variable with success probability $
%       h\lambda(ih-jh)$.
%     \item If $U_{ih}=1$:  
%       \begin{itemize}
%       \item[(i)] Simulate $X_{ih}=x_{ih}$ from $q(x_{jh},x_{ih},(i-j)b,\theta_j)$.
%       \item[(ii)] Update the weight
%         \[
%         w_{ih}=w_{jh}\rho_h(x_{(i-1)h},x_{ih},h;\theta_j,ih-jh),
%         \]
%       \item[(iii)] Set $j=i$; and choose an appropriate $\theta_j$ value.
%       \end{itemize}.
%     \end{enumerate}
%     \rule{\textwidth}{1mm}
%     \caption{\footnotesize SIS with Retrospective Sampling and Rao-Blackwellisation. \label{Alg:3}}
%   \end{footnotesize}
% \end{algorithm}

\subsection*{Continuous-time Importance Sampling}

Whilst Algorithm {\algrbsis} cannot be implemented, we can now take
the limit as $h\rightarrow0$. In doing this the Bernoulli random
variables will converge to a renewal process with rate of an event at
a time $\tau$ since the last event being $\lambda(\tau)$. We will thus
obtain a limiting algorithm where events are simulated from a Poisson
process, the value of the process at these events are drawn from the
proposal transition density, and the weights are updated based on the
simulated value. The key thing is that in this limit the incremental
weight is tractable. If we fix $s=jh$ and $t=ih$ and let $h\rightarrow
0$, then
% 
\begin{align*}
&\mrw{x_{s}}{x_{t}}{t-s}{\theta_s}:=\lim_{h\rightarrow 0}
\mrwh{x_{s}}{x_{t}}{h}{t-s}{\theta_s}\\
% 
&= 1 + \frac{1}{\lambda(t-s)} \lim_{h\rightarrow 0} \int
\frac{1}{h}\left\{\frac{\prd{x_{s}}{\y}{t-s-h}{\theta_s}[\trd{\y}{x_{t}}{h}-\prd{\y}{x_{t}}{h}{\theta_s}]}{\prd{x_{s}}{x_{t}}{t-s}{\theta_s}}\right\}\mbox{d}\y.
\end{align*}
% 
However by integrating (\ref{eq:PDE}) over a time interval of length
$h$, with an initial distribution for the process being $
\prd{x_{s}}{\y}{t-s-h}{\theta_s}$ we get:
% 
\begin{align*} \int
  \prd{x_{s}}{\y}{t-s-h}{\theta_s}\trd{\y}{x_{t}}{h}\mbox{d}\y &=
  \prd{x_{s}}{x_t}{t-s-h}{\theta_s} \\
  &+ h \tro\prd{x_{s}}{x_t}{t-s-h}{\theta_s}+o(h),
\end{align*}
% 
and similarly for the term which involves
$\prd{\y}{x_t}{h}{\theta_s}$. Thus
% 
\begin{align*} \mrw{x_{s}}{x_{t}}{t-s}{\theta_s}
=1+\frac{\lsb\tro-\prot{\theta_s}
\rsb \prd{x_{s}}{\y}{t-s}{\theta_s}|_{\y=x_t}}{\lambda(t-s)\prd{x_{s}}{x_{t}}{t-s}{\theta_s}}.
\end{align*}
% 
The resulting continuous-time importance sampling (CIS) algorithm is
given in Algorithm \algcis. If we stop the algorithm at an arbitrary
time $T$, we output a distribution for $x_T$ together with an
importance sampling weight. 

\begin{description}

\item[{\bf Algorithm \algcis}:] {\it Continuous-time Importance Sampling
    algorithm} (CIS).

\item[{\it Input}:] $T$ a time to stop and $x_0$ the initial value.

\item[{\it Initialise}:] Set $w_0=1,\,s=0$ and choose $\theta_0$.
  
\item[{\it Iterate}:] While $s<T$
  \begin{enumerate}
    
  \item draw $\tau$ the time until the next event in a Poisson process
    of rate $\lambda(\tau)$,
    
  \item if $s+\tau > T$, set $w_T=w_s$ and stop.
  \item\label{item:cis_update} Otherwise

    \begin{enumerate}
    \item set $t=s+\tau$,
    \item\label{item:cis_up_draw} draw $x_{t}\sim
    \prd{x_s}{\cdot}{t-s}{\theta_s}$,
  \item update the weight
    \begin{align*}
      w_t=w_s\,\mrw{x_s}{x_t}{t-s}{\theta_s},
    \end{align*}
  \item set $s=t$ and choose $\theta_s$.
    \end{enumerate}
  \end{enumerate}

\item[{\it Output}:] A distribution for the value of the process at
  time $T$, $\prd{x_s}{x_T}{T-s}{\theta_s}$, and a corresponding
  importance sampling weight $w_T$.

\end{description}



% \begin{algorithm}[ht]
%   \begin{footnotesize}
%     \rule{\textwidth}{1mm}
%     \underline{CIS.}

%     \begin{tabular}[h]{ll}
%       {\bf Input:} $T$ a time to stop.
%       \\
%       {\bf Initialise:} & Set $X_0=x_0$, $w_0=1$, $s=0$, and choose an appropriate $\theta_0$.
%       \\
%       \\ 
%     \end{tabular}

%     {\bf Iterate:} while $s<T$
%     \begin{enumerate}
%     \item Simulate $\tau$ the time until the next event in a Poisson process of rate $\lambda(\tau)$.
%     \item If $s+\tau>T$, set $t=T$, $w_T=w_s$, and  stop.  
%     \item Otherwise
%       \begin{itemize}
%       \item[(i)] Set $t=s+\tau$.
%       \item[(ii)] Simulate $x_{t}$ from $q(x_s,x_{t},t-s;\theta_s)$.
%       \item[(iii)] Update the weight
%         \[
%         w_{t}=w_s \rho_0(x_{s},x_{t},\theta_s,t-s).
%         \]
%       \item[(iv)] Set $s=t$, and choose an appropriate $\theta_s$. 
%       \end{itemize}
    % \end{enumerate}
%     {\bf Output:} A distribution for the value of the process at time $T$, $q(x_s,x_T,T-s;\theta-s)$, and a corresponding importance sampling weight $w_T$. \hfill
%     \rule{\textwidth}{1mm}
%     \caption{\footnotesize Continuous Importance Sampling (CIS) algorithm \label{Alg:4}}
%   \end{footnotesize}
% \end{algorithm}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> format.tex <==
\evensidemargin=-15pt
\oddsidemargin=0pt
\textwidth=460pt
\textheight=708pt
\voffset=-40pt
\setlength{\bibsep}{0.0pt}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> valid.tex <==
\section{Validity of CIS}\label{sec:validity-cis}

We will now consider the CIS algorithm directly, and show under what
conditions estimates of the form (\ref{eq:unbias}) are unbiased. To do
this we will first introduce some new notation. If we stop the CIS
algorithm at time $t$ we output a weight $w_t$ and a distribution
$q(\x_s,\x_t,t-s;\theta_s)$, where $s$ is the last Poisson event prior
to time $t$. With a slight abuse of notation we will denote the latter
by $q(\x_t;\beta_t)$. Thus $\beta_t$ contains all the information
about the distribution of $\X_t$ contained in the time of and the
value of the process at the last event time, and the choice of
parameter $\theta$ used.

Now for (\ref{eq:unbias}) to be an unbiased estimate we will need
% 
\begin{align*} \int f(\y) \trd{\x_0}{\y}{t}\mbox{d}\y =
\mbox{E}_q\left[W_t\int f(\y)q(\y;\beta_t)\mbox{d}\y \right],
\end{align*}
% 
where the former is the expectation of $f(\X_t)$ under the target
process, and the $\mbox{E}_q$ denotes the expectation with respect to
$W_t,\beta_t$ under the CIS process. Now assuming we can interchange
expectation and integration we have
% 
\begin{align*} \mbox{E}_q\left[W_t\int f(\y)q(\y;\beta_t)\mbox{d}\y
\right] = \int f(\y) \mbox{E}_q\left[W_t q(\y;\beta_t)\right]
\mbox{d}\y.
\end{align*}
% 
Thus, if $\ttrd{\x_0}{\y}{t}:=\mbox{E}_q\left[W_t
q(\y;\beta_t)\right]$, we will have unbiased estimates if
$\ttrd{\x_0}{\y}{t}=\trd{\x_0}{\y}{t}$. Note that we can view
$w_tq(\cdot;\beta_t)$ as an estimate of the transition density
$p(\x_0,\cdot,t)$, and thus $\tilde{p}(\x_0,\y,t)$ is just the
expectation of the corresponding estimator. Hence for CIS to produce
unbiased estimates,  we just need the estimate of
the transition density to be unbiased.

The key to showing when $\ttrd{\x_0}{\y}{t}=\trd{\x_0}{\y}{t}$ is the
following theorem.
% 
\begin{theorem} 
If $\mbox{E}(|W_t|)<\infty$ for all $t\leq T$. Then
for all $t \leq T$, $\tilde{p}(\x_0,\y,t)$ satisfies the following
differential equation
\begin{align*}
  \frac{\partial}{\partial t} \ttrd{\x_0}{\y}{t} =\tro 
\ttrd{\x_0}{\y}{t},
\end{align*}
% 
where $\tro$ is the forward operator of the target process,
defined in (\ref{eq:PDE}).
\end{theorem}

PROOF????

COMMENT ON INITIAL CONDITION IS CORRECT -- HENCE PROVIDING SOLUTION IS UNIQUE (REFS) THEN WE HAVE TILDEP=P.

FURTHER IMPORTANCE SAMPLING CORRECTION. GIVE ADAPTION TO CIS; LEMMA OF VALIDITY; AND OPTIMAL IS.

CAN WE SHOW THAT LAMBDA CAN DEPEND ON Xt PROVIDING WE CAN DO THE SIMULATION -- EG FOR THINNING??

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

